Boosting Deep Open World Recognition by Clustering

While convolutional neural networks have brought significant advances in robot vision, their ability is often limited to closed world scenarios, where the number of semantic concepts to be recognized is determined by the available training set. Since it is practically impossible to capture all possible semantic concepts present in the real world in a single training set, we need to break the closed world assumption, equipping our robot with the capability to act in an open world. To provide such ability, a robot vision system should be able to (i) identify whether an instance does not belong to the set of known categories (i.e. open set recognition), and (ii) extend its knowledge to learn new classes over time (i.e. incremental learning). In this work, we show how we can boost the performance of deep open world recognition algorithms by means of a new loss formulation enforcing a global to local clustering of class-specific features. In particular, a first loss term, i.e. global clustering, forces the network to map samples closer to the class centroid they belong to while the second one, local clustering, shapes the representation space in such a way that samples of the same class get closer in the representation space while pushing away neighbours belonging to other classes. Moreover, we propose a strategy to learn class-specific rejection thresholds, instead of heuristically estimating a single global threshold, as in previous works. Experiments on RGB-D Object and Core50 datasets show the effectiveness of our approach.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sections/tables.tex <==
\begin{table}[t]
\centering
\begin{tabular}{llllll}
\multicolumn{6}{c}{\textbf{Closed} World \textbf{without} rejection} \\ \hline
\multicolumn{1}{|l|}{METHOD} & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{Avg.} \\
\multicolumn{1}{|l|}{} & 11 & 16 & 21 & \multicolumn{1}{l|}{26} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{NNO} & \multicolumn{1}{l|}{76.7} & \multicolumn{1}{l|}{59.5} & \multicolumn{1}{l|}{51.6} & \multicolumn{1}{l|}{42.0} & \multicolumn{1}{l|}{57.5} \\ \hline
\multicolumn{1}{|l|}{Deep-NNO} & \multicolumn{1}{l|}{74.8} & \multicolumn{1}{l|}{64.5} & \multicolumn{1}{l|}{61.4} & \multicolumn{1}{l|}{55.3} & \multicolumn{1}{l|}{64.0} \\ \hline
\multicolumn{1}{|l|}{Ours} & \multicolumn{1}{l|}{78.6} & \multicolumn{1}{l|}{67.9} & \multicolumn{1}{l|}{66.4} & \multicolumn{1}{l|}{60.3} & \multicolumn{1}{l|}{68.3} \\ \hline
\end{tabular}
\caption{Results of closed world with rejection. The model is incrementally tested only on known classes.}
\label{tab:without_rejection}
\end{table}


\begin{table}[t]
\centering
\begin{tabular}{llllll}
\multicolumn{6}{c}{\textbf{Closed} World \textbf{with} rejection} \\ \hline
\multicolumn{1}{|l|}{METHOD} & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{Avg.} \\
\multicolumn{1}{|l|}{} & 11 & 16 & 21 & \multicolumn{1}{l|}{26} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{NNO} & \multicolumn{1}{l|}{30.6} & \multicolumn{1}{l|}{22.1} & \multicolumn{1}{l|}{18.2} & \multicolumn{1}{l|}{14.7} & \multicolumn{1}{l|}{21.4} \\ \hline
\multicolumn{1}{|l|}{Deep-NNO} & \multicolumn{1}{l|}{46.2} & \multicolumn{1}{l|}{48.3} & \multicolumn{1}{l|}{48.4} & \multicolumn{1}{l|}{43.0} & \multicolumn{1}{l|}{46.5} \\ \hline
\multicolumn{1}{|l|}{Ours} & \multicolumn{1}{l|}{58.1} & \multicolumn{1}{l|}{54.0} & \multicolumn{1}{l|}{49.3} & \multicolumn{1}{l|}{40.8} & \multicolumn{1}{l|}{50.5} \\ \hline
\end{tabular}
\caption{Results of closed world with rejection. The model is incrementally tested only on known classes plus the possibility to predict also a single unknown class.}
\label{tab:with_rejection}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{llllll}
\multicolumn{6}{c}{\textbf{Open Set} recognition} \\ \hline
\multicolumn{1}{|l|}{METHOD} & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{Avg.} \\
\multicolumn{1}{|l|}{} & 11 & 16 & 21 & \multicolumn{1}{l|}{26} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{NNO} & \multicolumn{1}{l|}{94.8} & \multicolumn{1}{l|}{94.3} & \multicolumn{1}{l|}{93.2} & \multicolumn{1}{l|}{92.4} & \multicolumn{1}{l|}{93.7} \\ \hline
\multicolumn{1}{|l|}{Deep-NNO} & \multicolumn{1}{l|}{86.5} & \multicolumn{1}{l|}{70.9} & \multicolumn{1}{l|}{60.9} & \multicolumn{1}{l|}{58.4} & \multicolumn{1}{l|}{69.2} \\ \hline
\multicolumn{1}{|l|}{Ours} & \multicolumn{1}{l|}{73.2} & \multicolumn{1}{l|}{67.4} & \multicolumn{1}{l|}{72.3} & \multicolumn{1}{l|}{73.8} & \multicolumn{1}{l|}{71.7} \\ \hline
\end{tabular}
\label{tab:open_set}
\caption{Results of open set. The model is incrementally tested only on unknown classes.}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{lllllll}
\multicolumn{7}{c}{\textbf{Open World} recognition} \\ \hline
\multicolumn{1}{|l|}{METHOD} & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{Avg.} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Harm. \\ Avg.\end{tabular}} \\
\multicolumn{1}{|l|}{} & 11 & 16 & 21 & \multicolumn{1}{l|}{26} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{NNO} & \multicolumn{1}{l|}{62.7} & \multicolumn{1}{l|}{58.2} & \multicolumn{1}{l|}{55.7} & \multicolumn{1}{l|}{53.5} & \multicolumn{1}{l|}{57.5} & \multicolumn{1}{l|}{34.8} \\ \hline
\multicolumn{1}{|l|}{Deep-NNO} & \multicolumn{1}{l|}{66.4} & \multicolumn{1}{l|}{59.6} & \multicolumn{1}{l|}{54.7} & \multicolumn{1}{l|}{50.7} & \multicolumn{1}{l|}{57.8} & \multicolumn{1}{l|}{55.6} \\ \hline
\multicolumn{1}{|l|}{Ours} & \multicolumn{1}{l|}{65.7} & \multicolumn{1}{l|}{60.7} & \multicolumn{1}{l|}{60.8} & \multicolumn{1}{l|}{57.3} & \multicolumn{1}{l|}{\textbf{61.1}} & \multicolumn{1}{l|}{\textbf{59.3}} \\ \hline
\end{tabular}
\caption{Results of open world recognition. The model is incrementally tested on known and unknown classes.}
\label{tab:open_world}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{lllllll}
\multicolumn{7}{c}{\textbf{Clustering ablation}} \\ \hline
\multicolumn{1}{|l|}{METHOD} & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{Avg.} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Harm. \\ Avg.\end{tabular}} \\
\multicolumn{1}{|l|}{} & 11 & 16 & 21 & \multicolumn{1}{l|}{26} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{GC + LC} & \multicolumn{1}{l|}{67.7} & \multicolumn{1}{l|}{59.6} & \multicolumn{1}{l|}{59.5} & \multicolumn{1}{l|}{57.3} & \multicolumn{1}{l|}{\textbf{61.0}} & \multicolumn{1}{l|}{\textbf{60.8}} \\ \hline
\multicolumn{1}{|l|}{GC} & \multicolumn{1}{l|}{66.0} & \multicolumn{1}{l|}{57.3} & \multicolumn{1}{l|}{58.6} & \multicolumn{1}{l|}{53.3} & \multicolumn{1}{l|}{58.8} & \multicolumn{1}{l|}{58.7} \\ \hline
\multicolumn{1}{|l|}{LC} & \multicolumn{1}{l|}{64.1} & \multicolumn{1}{l|}{56.0} & \multicolumn{1}{l|}{57.9} & \multicolumn{1}{l|}{56.4} & \multicolumn{1}{l|}{58.6} & \multicolumn{1}{l|}{58.4} \\ \hline
\end{tabular}
\caption{Ablation of clustering techniques.}
\label{tab:ablation_clustering}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{llll}
\multicolumn{4}{c}{\textbf{Rejection rates}} \\ \hline
\multicolumn{1}{|l|}{Method} & \multicolumn{1}{l|}{Known} & \multicolumn{1}{l|}{Unknown} & \multicolumn{1}{l|}{Difference} \\ \hline
\multicolumn{1}{|l|}{Our tau} & \multicolumn{1}{l|}{27.4} & \multicolumn{1}{l|}{65.2} & \multicolumn{1}{l|}{\textbf{37.8}} \\ \hline
\multicolumn{1}{|l|}{Deep-NNO tau} & \multicolumn{1}{l|}{4.4} & \multicolumn{1}{l|}{26.9} & \multicolumn{1}{l|}{22.6} \\ \hline
\multicolumn{1}{|l|}{NNO tau} & \multicolumn{1}{l|}{84.4} & \multicolumn{1}{l|}{98.8} & \multicolumn{1}{l|}{14.4} \\ \hline
\end{tabular}
\caption{Rajection rates of different techniques for detecting the unknowns.}
\label{tab:ablation_unknown}
\end{table}
